Shape-Biased Domain Generalization via Shock Graph Embeddings

There is an emerging sense that the vulnerability of Image Convolutional Neural Networks (CNN), i.e., sensitivity to image corruptions, perturbations, and adversarial attacks, is connected with Texture Bias. This relative lack of Shape Bias is also responsible for poor performance in Domain Generalization (DG). The inclusion of a role of shape alleviates these vulnerabilities and some approaches have achieved this by training on negative images, images endowed with edge maps, or images with conflicting shape and texture information. This paper advocates an explicit and complete representation of shape using a classical computer vision approach, namely, representing the shape content of an image with the shock graph of its contour map. The resulting graph and its descriptor is a complete representation of contour content and is classified using recent Graph Neural Network (GNN) methods. The experimental results on three domain shift datasets, Colored MNIST, PACS, and VLCS demonstrate that even without using appearance the shape-based approach exceeds classical Image CNN based methods in domain generalization.

==> shock_compute.tex <==
\section{Shock Graph Computational Algorithm}


Formally, the computation of shocks from an unorganized set of curve fragments relies on two key ideas. First, since the shocks arising from points and lines can be analytically computed, the curve fragments can be first approximated by a polyline, namely, a set of line segments that share end points; there are well-known algorithms to achieve this by specifying the expected error~\cite{vxl:webcite}. It is well-known that the bisector of two points is a line, the bisector of two lines is a line, and the bisector of a point and a line is a parabola, Figure~\ref{fig:bisect}. The dynamics of shocks moving on this bisector are less trivial but they can also be calculated analytically. The geometry and dynamics of shocks arising from any isolated pair from a collection of point and line sources is therefore readily available in analytic form and this saves in computation time and provides numerical stability robustness. 

\begin{figure}[ht]
\center
a)\includegraphics[width=0.221\textwidth]{figs/point-point-fixed.pdf}
b)\includegraphics[width=0.4\textwidth]{figs/line-line-fixed.pdf}
c)\includegraphics[width=0.221\textwidth]{figs/point-line-fixed.pdf}

\caption{Analytic computation of shocks from polylines requires shocks from (a) point-point (b) line-line and (c) point-line pairs. Boundary “sources” are shown in red, shocks are shown in green, and the rays connecting boundary sources to respective shocks are shown in dashed lines. These computations assume only a pair of sources with no interaction from other sources so all shocks go off to infinity.  } 
\label{fig:bisect}
\end{figure}

The second key idea is the use of a wave propagation and shock propagation to piece together shocks from multiple pairs of sources in a highly efficient way. Observe that the union of all shock-graph of isolated pairs of sources is a superset of the shock graph of the union of boundary sources, \eg, as in the bisectors shown in grey and green which is a superset of the shock graph shown in green in Figure~\ref{fig:sc2_steps}{(h)}. Consider first the shock points on a bisector of a pair of boundary sources: a shock point is valid if no other waves from sources other than its own sources reach there. In other words, a shock is valid if its time of formation (distance to its sources) is earlier than the time of propagation (distance) to any earlier other source. Since the shock path on any bisector has an initial shock point (shock source), the extent of the valid shock path can be determined by first examining the validity of the shock source itself, the first shock point to form in time. Since a valid shock path can only be potentially terminated at the intersection of two shock paths, these are the only points that need to be examined. This is a key distinction since it discretizes the continuous propagation into a discrete propagation. Thus, the algorithm first computes all shock sources, an $N^2$ computation for $N$ boundary sources, and considers shock paths for the sources in order of time. 

\begin{figure*}[ht]
\center
{\footnotesize\textit{a}}\includegraphics[width=0.235\textwidth]{figs/incremental-voro-02-01.pdf}
{\footnotesize\textit{b}}\includegraphics[width=0.235\textwidth]{figs/incremental-voro-02-02.pdf}
{\footnotesize\textit{c}}\includegraphics[width=0.235\textwidth]{figs/incremental-voro-03-01.pdf}
{\footnotesize\textit{d}}\includegraphics[width=0.235\textwidth]{figs/incremental-voro-03-02.pdf}
{\footnotesize\textit{e}}\includegraphics[width=0.235\textwidth]{figs/incremental-voro-04-01.pdf}
{\footnotesize\textit{f}}\includegraphics[width=0.235\textwidth]{figs/incremental-voro-04-02.pdf}
{\footnotesize\textit{g}}\includegraphics[width=0.235\textwidth]{figs/incremental-voro-05-01.pdf}
{\footnotesize\textit{h}}\includegraphics[width=0.235\textwidth]{figs/incremental-voro-05-02.pdf}

\caption{This figure illustrates the incremental steps of shock computation for a set of \textcolor{red}{red input curves}. At each step infinite length \textcolor{cyan}{cyan bisector curves} between a new boundary element and each of the previous boundary elements are computed. The finite true bisectors after the limiting process are shown in \textcolor{green}{green} with the removed shock branches shown in \textcolor{gray}{gray}. The \textcolor{green}{green shock links} represent the valid portion of bisector curves.} 
\label{fig:sc2_steps}
\end{figure*}


Figure~\ref{fig:sc2_steps} illustrates this process. Consider two fragments, $C_1$ and $C_2$ whose potential shock path is shown in cyan in (a).  For the purpose of illustrating the second key idea, namely using propagation to compute the shock graph, the contour fragments are not restricted to be polylines and can take any form. Also, these are sketches and not accurate in scale. Since there are no other interacting shock paths, the entire shock path is validated and shown in green. Next, suppose that a third contour fragment $C_3$ is added to the pool of curve fragments. The interaction of the new-comer $C_3$ with $C_1$ and $C_2$ generates two potential shock paths shown in cyan in (c). The intersection of these shock paths with existing shock paths create shock junctions, which are the only potential terminators of a shock path. In this particular case there is only one shock junction, with each of the three shock paths flowing into the shock junction. Since the continuation of each shock path has a time exceeding the time of the waves reaching there from another source, all three shock paths are terminated, as shown in (d). In other cases it can happen that two shock branches flow into a junction and one shock branch flows out. In this case the two branches flowing into the junction are terminated in which the shock branch flowing out only begins at the junction as its source. It can also happen that the entire shock path is invalid, say if the two sources on the opposite sides of an image with many sources in between. Consider now $N$ boundary sources. The process of shock computation can be implemented by first computing the shock path for a pair of boundary sources, and then considering a third, a fourth, \etc. , Figure~\ref{fig:sc2_steps}. While this can be done in any order, the most efficient order is one that considers the earliest forming shocks first. 



The practical implementation of these two ideas is realized through the construction and visitation of two time-ordered lists. The first list contains the \emph{candidate} sources that are initially pre-computed and has size $N^2$ and is a superset of all possible source nodes in the shock-graph. The second list is the \emph{active} shock list, the list of shocks under propagation, and is initially empty. The algorithm proceeds by visiting the first element in the \emph{candidate} source list and initializing a pair of child shocks (outgoing flow) where each child has a start time equivalent to the time of formation of the source node and an end time initially at infinity. This initial pair of shocks are inserted into the active elements list, and the source node is removed from the \emph{candidate} list. Each \emph{active} shock is then propagated to the nearest junction on it, thus forming a valid shock link of the shock graph, with a specific start and a specific end-time, and this active shock is now removed from the list. The process is iterated by visiting the next active shock in the list. As the algorithm alternates between visiting the two lists it prioritizes visiting \emph{active} shock elements first over candidate sources. If there are no more active shocks the algorithm will visit the next element in the candidate source list, initialize a new pair of child shocks, and subsequently propagate those active shocks to determine junctions with the existing shocks. This process will terminate when both lists are empty. As candidate sources are visited the algorithm determines which sources are valid or invalid given the current state of the simulation, before initializing a new pair of child shocks. It is formally shown in~\cite{Tamrakar:Kimia:Shock} that the number of discarded candidate sources in the second stage (propagation of shocks) leads to a logarithmic dependency on the number of contours, $N$, resulting in an overall run-time of $N^2log(N)$. Note that during this process, shocks, shock nodes, and shock links are augmented with continuous attributes such as its intrinsic geometry (time of formation, length, curvature, \etc) and also labeled with discrete attributes signifying the \emph{node type}, namely, source, sink, or junction and \emph{link type}, namely, degenerate, semi-degenerate, or degenerate~\cite{Giblin:Kimia:IJCV03}. 









%% and inserts these shocks 

%% each of the $N^2$ candidate sources sequentially, initializes a pair of outgoing (child) shocks from the source node, and subsequently inserts them into the \emph{active} shocks list.   If all active shocks are extinguished then the next 

%% If the wavefronts are quenched for that shock path, then the next candidate source is visited in the time-ordered list. If however, the interaction of the shock path with other sources causes a new shock path to arise then that new element is reinserted into the list with the appropriate time. This process terminates when the list is exhausted. The final result of this second stage is the formation of a set of shock links and shock nodes. The intersection of shock paths or bisector curves creates new shock nodes that are shock junctions.  The formation of shock nodes, limits each shock path to its valid portion of the bisector curve, which we refer to as shock links or shock segments. Shock links capture the relationship between nodes and are directed from newer to older, according to the time of formation of the nodes in the curve evolution process. The set of shock nodes and the connecting shock segments defines a shock graph.






%% \begin{figure*}[ht]
%% \center
%% a)\includegraphics[width=0.22\textwidth]{figs/sc2_step_1.pdf}
%% b)\includegraphics[width=0.22\textwidth]{figs/sc2_step_2.pdf}
%% c)\includegraphics[width=0.22\textwidth]{figs/sc2_step_3.pdf}
%% d)\includegraphics[width=0.22\textwidth]{figs/sc2_step_4.pdf}
%% \caption{A \textcolor{red}{contour} represented by a set of polylines. In a) we see how two adjacent polylines spawn a bisector (dashed \textcolor{green}{- -} line). Subsequent steps b)c) and d) determine the valid portion (solid \textcolor{green}{-} line ) of each bisector curve. Also notice the formation of shock nodes at the intersection of bisector curves. } 
%% \label{fig:sc2_steps}
%% \end{figure*}



%% Formally the shock computation algorithm consists of two stages. Given an input of an unorganized set of contours, approximated by discrete polylines, a set of continuous exact candidate shock paths are analytically computed between all pairs of contour elements (points or lines), Figure~\ref{fig:bisect}. The shock segment lies on the bisector curve of a pair of contour elements augmented with the dynamics of flow corresponding to when the wave-fronts from the two sources come together, the instantaneous velocity of shock points along the curve, and the direction of monotonic flow along the curve.  This refinement of a medial-axis segment to a shock path  The output of the first stage is a set of $N^2$, where $N$ is the number of polyline segments, candidate shock paths of infinite length that are pruned in subsequent stages. A list is maintained of these candidate shock paths that is ordered according to time of formation \ie minimum distance between two boundary elements. 
 
%%  Since the interaction of two sources can be fully invalidated or spatially limited by the presence of other sources, in a second stage, all combinations of shock paths are considered to explore this effect, Figure~\ref{fig:sc2_steps}. 



%% \begin{figure}[ht]
%% \center
%% \includegraphics[width=0.4\textwidth]{figs/shock_computation.pdf}
%% \caption{A set of curves in black and all pairs of bisectors shaded out in gray. The blue curves or shocks represent the valid portions of bisector curves.} 
%% \label{fig:shock_compute}
%% \end{figure}

 


Finally, there are two practical considerations in utilizing the shock computation algorithm of~\cite{Tamrakar:Kimia:Shock}. First, many shock paths extend infinitely beyond the image borders. The addition of a bounding box to the initial set of contour fragments contains the shock paths to a finite, well-defined area. In practice, this bounding box is twice the size of the image, Figure~\ref{fig:shocks_regular}. Second, the approximation of each contour fragment as a polyline generates numerous artifactual shocks at the points of convex discontinuity. The regularization algorithm in~\cite{Tamrakar:Kimia:Shock} recovers the ``true'' shock graph, Figure~\ref{fig:shocks_regular}, \ie, the shock graph of the contour before the polyline approximation, by scoring and removing shock links according to some user-defined threshold. The saliency computed for each shock link measures the amount of deformation of the boundary that is needed for the link to be removed. It is closely related to the ``splice cost'' in~\cite{Sebastian:etal:Shocks:PAMI2004}. In all subsequent figures, unless otherwise noted, the shock computation is depicted with a bounding box twice the size of the image and with $\lambda=1.0$ regularization.  

\begin{figure}[ht]
\centering
{\footnotesize\textit{a}}\includegraphics[width=0.22\textwidth]{figs/calf_nobbox_noreg.pdf}
{\footnotesize\textit{b}}\includegraphics[width=0.22\textwidth]{figs/calf_bbox_reg.pdf}
\caption{a) The set of \textcolor{red}{red contours} and its corresponding shock graph in \textcolor{green}{green}. b) If we augment the contour set with a \textcolor{magenta}{magenta} bounding box and apply regularization ($\lambda=1.0$) we recover the shock graph corresponding to the initial contour, before the polyline approximation. }
\label{fig:shocks_regular}
\end{figure}



